Operational State Complexity of Deterministic Unranked Tree Automata

We consider the state complexity of basic operations on tree languages recognized by deterministic unranked tree automata. For the operations of union and intersection the upper and lower bounds of both weakly and strongly deterministic tree automata are obtained. For tree concatenation we establish a tight upper bound that is of a different order than the known state complexity of concatenation of regular string languages. We show that (n+1) ( (m+1)2^n-2^(n-1) )-1 vertical states are sufficient, and necessary in the worst case, to recognize the concatenation of tree languages recognized by (strongly or weakly) deterministic automata with, respectively, m and n vertical states.

==> eptcsdata.tex <==
\providecommand{\firstpage}{149}
\providecommand{\publicationstatus}{I. McQuillan and G. Pighizzini (Eds.): 12th International Workshop\\on Descriptional Complexity of Formal Systems (DCFS 2010)\\
EPTCS 31, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.31.17}{10.4204/EPTCS.31.17}}

